Wizundry: A Cooperative Wizard of Oz Platform for Simulating Future Speech-based Interfaces with Multiple Wizards

Wizard of Oz (WoZ) as a prototyping method has been used to simulate intelligent user interfaces, particularly for speech-based systems. However, as our societies' expectations on artificial intelligence (AI) grows, the question remains whether a single Wizard is sufficient for it to simulate smarter systems and more complex interactions. Optimistic visions of 'what artificial intelligence (AI) can do' places demands on WoZ platforms to simulate smarter systems and more complex interactions. This raises the question of whether the typical approach of employing a single Wizard is sufficient. Moreover, while existing work has employed multiple Wizards in WoZ studies, a multi-Wizard approach has not been systematically studied in terms of feasibility, effectiveness, and challenges. We offer Wizundry, a real-time, web-based WoZ platform that allows multiple Wizards to collaboratively operate a speech-to-text based system remotely. We outline the design and technical specifications of our open-source platform, which we iterated over two design phases. We report on two studies in which participant-Wizards were tasked with negotiating how to cooperatively simulate an interface that can handle natural speech for dictation and text editing as well as other intelligent text processing tasks. We offer qualitative findings on the Multi-Wizard experience for Dyads and Triads of Wizards. Our findings reveal the promises and challenges of the multi-Wizard approach and open up new research questions.

==> design.tex <==
\section{System Design of Wizundry}
Wizundry is a web application for solo or multi-Wizard WoZ experiments.
We used followed several literature-informed design considerations so as to allow experimenters to easily and rapidly conduct WoZ experiments. The tool features role-based experimentation capabilities for explicitly separating the functionality to be implemented by individual roles in multi-Wizards experiments.


\subsection{Design Considerations}
We developed Wizundry for the voice interaction scenario of speech dictation. We considered several factors involved in supporting multi-Wizard collaboration within this context of use. These were established based on existing WoZ tools \cite{10.1145/3386867,10.1145/169059.169215,10.1145/3405755.3406148,10.1145/3343413.3377941,schlogl2013webwoz} and explorations of the Wizard experience \cite{8673205,10.1145/1452392.1452419,10.1145/3027063.3053175}. The key considerations were as follows:

\begin{itemize}
    \item[-] Short learning curve and an easy-to-use tool that can be used by multiple Wizards at the same time.
    \item[-] Empathizing with the Wizard and designing from the point of view of the Wizard as an essential user.
    \item[-] Flexible for use in a wide range of remote and cross-device scenarios, with minimal dependency on application platforms and devices.
    \item[-] Provide a fast and efficient research tool for researchers who need to use WoZ in their work.
    \item[-] Using component-based development so that experimenters can choose which features to enable based on the needs of each experiment.
    \item[-] Using sockets to connect all Wizards in real-time to achieve transparent and efficient division of labour and provide a better user experience for all users.
    
\end{itemize}

%Wizundry was designed with these key features. 
The following sections detail the design of the system and how it is used.


\subsection{System Features}
The Wizundry platform has several features and functions for the experimenter to choose among based on their own needs. There are two core features that rely on Natural Language Processing (NLP) and collaborative techniques. For the NLP, we implemented Mozilla Web Speech API \footnote{See https://developer.mozilla.org/en-US/docs/Web/API/Web\_Speech\_API} and Google Cloud Speech API \footnote{See https://cloud.google.com/speech-to-text}. NLP was used for generating speech-to-text (STT) in the command boxes, speech recognition, microphone, and editor content playback. For the collaborative function, we used socket.io\footnote{See https://socket.io/}, Yjs\footnote{See https://github.com/yjs/yjs}, tiptap editor\footnote{See https://www.tiptap.dev/}, and web-socket to realize the real-time collaborative editor, cursor, and name flag features. Fig.\ref{fig.strategy} shows the collaborative features and methodology.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=1.0\linewidth]{Figure/Socket Collaboration.png}
  \caption{All collaborative techniques and implementation}
  \label{fig.strategy}
\end{figure}


\subsubsection{Collaborative Editor and Name Flag}
The collaborative editor allows multiple Wizards to cooperate at the same time, with the user (Fig.\ref{Fig.Wizard}.e). Much of the WoZ literature underlined the importance of system transparency for the user. In cooperative contexts, explanations for and visibility of others' actions allow people to feel greater confidence in the system. To this end, we designed a “name flag” similar to the Google Docs approach (Fig.\ref{Fig.Wizard}.f). The flag will display as a pop-up over the current position of the Wizard's cursor while the other Wizard/s are editing the content.

Each Wizard can view the other Wizard/s' cursor/s in real-time (Fig.\ref{Fig.Wizard}.g). In the example illustrated in Fig.\ref{Fig.Wizard}.g, the green cursor belongs to another Wizard. We also provided shortcut keys for the common functions that Wizards frequently use (Fig.\ref{Fig.Wizard}.b). For instance, Wizards can press Ctrl/Cmd+Q to control the microphone.

\subsubsection{Collaborative Cursor}
In a collaborative tool, it is convenient and effective to provide each other's digital position in real-time as an indicator of presence and to reduce conflicts. Showing the cursor can help each Wizard complete solo and shared tasks and locate each other in the interface \cite{fussell2003assessing} while increasing the transparency of the their own actions and the efficiency of collaboration \cite{alem2011study}. Wizundry listens to the cursor movement event after two Wizards have entered the same socket room, and immediately sends the coordinates (clientX, clientY) to the other Wizard. When a new Wizard joins, a cursor id is created based on the Wizard name to distinguish it.

\subsubsection{Speech Recognition and Microphone Control}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.6\linewidth]{Figure/Speech-to-Text.png}
%   \caption{Microphone Control and Google Cloud Speech-to-Text Implementation}
%   \label{fig.speech-to-text}
% \end{figure}
% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.6\linewidth]{Figure/Text-to-Speech.png}
%   \caption{Speaker Control and Web Speech Synthesis Implementation}
%   \label{fig.text-to-speech}
% \end{figure}


\begin{figure}[htbp]
  \centering
  \includegraphics[width=1.0\linewidth]{Figure/wireframe.png}
  \caption{(1) Microphone Control and Google Cloud Speech-to-Text Implementation; (2) Speaker Control and Web Speech Synthesis Implementation;}
  \label{fig.wireframe}
\end{figure}


%
%\begin{figure}[htbp]
%  \centering
% \begin{minipage}[t]{0.48\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{Figure/Speech-to-Text.png}
%   \caption{Microphone Control and Google Cloud Speech-to-Text Implementation}
%   \label{fig.speech-to-text}
%  \end{minipage}
%  \begin{minipage}[t]{0.48\textwidth}
%    \centering
%    \includegraphics[width=1\linewidth]{Figure/Text-to-Speech.png}
%    \caption{Speaker Control and Web Speech Synthesis Implementation}
%    \label{fig.text-to-speech}
%  \end{minipage}
%\end{figure}

Due to recent advances in speech recognition, it is no longer necessary to use an unnatural sound effect as a cue for the user to reduce their composing speed so that the "Typewriter" \cite{10.1145/2163.358100} has enough time to hear and write what they say. Although this technology is still mechanized and prone to error, it makes some tasks easier for Wizardry, in particular dictation and translation tasks. Wizundry uses the Mozilla Web Audio Context\footnote{See https://developer.mozilla.org/en-US/docs/Web/API/AudioContext} to create a script processor, which handles the end-user's speech and encodes it in binary format. After transmitting the audio byte file from the front-end to the server, the Google Cloud Speech-to-Text API transforms the audio to text and transmits back to all users in the socket room (Fig.\ref{fig.wireframe}.1). Wizards can control the on/off status of the user's microphone by clicking the mic icon (Fig.\ref{Fig.Wizard}.c). The user cannot control the mic, but they can view its status (Fig.\ref{Fig.user}.c). We designed "open/closed" icon and color effects for the microphone to ensure that the Wizards and the user understand its status clearly(Fig.\ref{Fig.dictation}.1).

\subsubsection{Command Boxes}

Natural conversation is the most important part of the user experience in voice interaction. A core question when developing these platforms is: What is the most natural way of facilitating human-agent conversation, while maintaining consistency across Wizards? Thus we provided a series of static and editable conversation boxes that help each Wizard converse quickly so as to maintain a natural flow of conversation with the user. (Fig.\ref{Fig.Wizard}.d) There are two types of boxes, each with a different function; see (Fig.\ref{Fig.dictation}.2) for an illustration of the different states possible for these boxes. The white boxes are editable and will clear the content entered by the Wizard right after it is sent. This is to account for the possible situation that the Wizard would like to send a customize message only at once. The green boxes, however, are static, and will save the content so that the Wizards can repeat common responses, such as "Pardon?" and "Can you speak slowly?" Both types of boxes otherwise operate the same way: clicking the play button or hitting "Enter" on the keyboard converts the text input to audio, which is immediately played on the user's side. We used the Mozilla Web Speech Synthesis API and Web Speech Synthesis Utterance to carry out this feature (Fig.\ref{fig.wireframe}.2).


\subsubsection{Content Playback}
For a better user experience on editing the composed verbalization content, Wizundry provides a feature for the Wizard to play back the content for the end-user with the utilization of Web Speech Synthesis API. This feature cues the end-user to check the correctness of the post content without having to visually examine the screen. It also cues all parties to locate the content that needs to be corrected. This feature is triggered by the Wizard situating the mouse at the commencement of the verbalize back and pressing the ESC key, Web Speech Synthesis Utterance will cull the commencement to the cessation of the text as the content to be verbalized. The system will keep playing the sound until the next time the Wizard presses the ESC key or the content ends.

\subsubsection{Line Break and Punctuation}
The primary goal of applying layout to a text is to arrange it in such a way that it is easier to read and comprehend. The most straightforward method is to utilize punctuation and line breaks. \cite{hodel2004supporting} Wizundry adds punctuation characters and an invisible line break behind each line of the end-user composition. The readability of a document can already be significantly improved with these two techniques. Another benefit is that if the sentence contains complex ideas with many sub-clauses, branching can make it easier to understand and therefore quicker for both the Wizard/s and the end-user to comprehend, thus avoiding unnecessary re-flows associated with line wrapping \cite{himmelstein2019open}. In addition, line breaks can be utilized as a situating implement, allowing the Wizard to use the number of lines to determine where the user needs to edit the content effectively.

\subsubsection{Cross-Platform Application}
We have implemented our system as a web application that can operate on multiple platforms. Web applications can be deployed in the public domain and fortified with a high caliber of compatibility for operation in a variety of systems. We expect that our system can be used various kinds of studies, where experimenters decide whether to employ platforms such as tablets, personal computers, and smartphones. The most important part is that multiple Wizards and users can be located in different rooms without perturbing others.

\subsubsection{Role-based Authentication}
Considering that Wizundry is a web-based system, it is essential to protect the experimental data and enhance the platform's security. Therefore, Wizundry uses the JWT token authentication and further makes a role-based authentication to enhance the authenticity of client \cite{ahmed2019authentication}. With role-based login, roles are related to their corresponding functions and privileges. This protection allows only those who have the password to log in and participate in the experiment, and screen out malicious clients. The advantage of using JWT token is that the same user can use this token to log in quickly next time if the token has not expired, improving the efficiency of the experiment.

\subsubsection{Logs Storage}
In addition to the basic screen recordings and experimenter records, Wizundry also provides automatic logging to record Wizard and end-user operations in chronological order and each Trial ID for future quantitative Study and data analysis after the experiment is completed. It also records the text composition of the user and the opening and closing time of the experiment. It also records the user's text composition and the opening and closing time of the experiment. The information about the operator, the time, the content of the operation, the type of operation, etc. is recorded in the database.

%\begin{figure}[htbp]
%  \centering
%  \includegraphics[width=0.8\linewidth]{Figure/woz-logs.png}
%  \caption{experiment logs downloaded from the database with .csv format}
%  \label{fig.logs}
%\end{figure}

\subsection{Role-Based Components}
The Wizundry system can be divided into three roles: 1) the admin, which is the experimenter, 2) the Wizard, and 3) the end-user. Different functions and interface features are available according to these roles. Generally, the admin has the maximum ascendancy and can access the database, while Wizard and end-user have equal access levels but are presented with different interfaces that have different operation functions.

\begin{itemize}
\item[-] \textbf{Wizard Component}:
    The Wizard's interface consists of four components. The first is Command Boxes (See 3.3.4), which support editable responses. At the corner of left-top, a legend explaining interface shortcut keys is provided. The Microphone Control (See 3.3.3) is near the board; the status of mic is the same on every Wizard's interface. The Collaborative Editor on the right side is the largest and most important component (See 3.3.1). Name Flag and visible Cursor are displayed in real-time while a Wizard is editing content.
    \begin{figure}[htbp]
      \centering
      \includegraphics[width=1.0\linewidth]{Figure/Wizard_UI.png}
      \caption{The Wizard's interface. (b) Legend explaining interface shortcut keys. (c) Microphone control and status. (d) Editable command boxes. (e) Collaborative Editor. (f) Name flag. (g) Collaborative Cursor.}
      \label{Fig.Wizard}
    \end{figure}
    \begin{figure}[htbp]
      \centering
      \includegraphics[width=1.0\linewidth]{Figure/dictation.png}
      \caption{Illustration of the different possible states for the mic and speaker components. (1a) Mic is closed. (1b) Mic is opened. (2a) Default boxes, where white is cleared after sending and green is static, retaining the text. (2b) Custom input, where the Wizard hit "Enter" or click the button to save and send the command. (2c) After playing the command, the editable white box will clear but the static green box will retain.}
      \label{Fig.dictation}
    \end{figure}
\item[-] \textbf{End-User}:
    In real usage scenarios for dictation and other speech-based tasks, the end-user may not need to look at anything: they can rely on speech interaction, hand- and eye-free. But for composition tasks and lab testing, an end-user interface may be useful. The end-user interface in Wizundry is depicted in Fig.\ref{Fig.user}.  
    In comparison to the Wizard interface, the microphone button is inactive, because end-users cannot control it (Fig.\ref{Fig.user}.c). However, they can know whether the microphone is active or not through the status depicted by the microphone icon. End-users are provided with the editor without collaborative features, which demonstrates the composition of their dictation and the edited content from Wizards in real-time (Fig.\ref{Fig.user}.e).
    \begin{figure}[htbp]
      \centering
      \includegraphics[width=1.0\linewidth]{Figure/user_UI.png}
      \caption{The end-user's interface. (c) The user can see the status of the mic and is not allowed to control it. (e) The Collaborative Editor from the end-user's perspective. Notice that the Wizards' cursors, name tags, and cursor highlights are not visible.}
      \label{Fig.user}
    \end{figure}
\item[-] \textbf{Experimenter (Admin)}:
    In many WoZ experiments, the experimenter/s take on the role of observer. The purpose is to be able to control unexpected situations and record observations of the experiment. Thus, Wizundry provides an Admin role whereby the experimenter can monitor the experiment from another computer remotely without affecting the experiment. The Admin can select different trials (Fig.\ref{Fig.create}.1) according to the features required by each experiment (Fig.\ref{Fig.create}.2) before the experiment commences. (Fig.\ref{Fig.create}.3). After the trial is created, the Wizard/s and end-user can go to different breakout rooms and conduct the experiment independently according to the trial ID. (Fig.\ref{Fig.manage}.1) In other words, it is possible to conduct multiple multi-Wizard or single-Wizard experiments at the same time in Wizundry, because the data transfer between trial rooms will not affect each other. The Admin can also extract and download (Fig.\ref{Fig.manage}.3) the experiment logs as a .csv file (Fig.\ref{fig.logs}) on each trial from the database after the experiment is consummated.
    \begin{figure}[htbp]
      \centering
      \includegraphics[width=0.8\linewidth]{Figure/admin_create.png}
      \caption{The administrator's interface. (1) The administrator needs to enter necessary information to create a new experiment. (2) Administrator needs to select features that the new experiment will have. (3) Buttons for more actions.}
      \label{Fig.create}
    \end{figure}
    \begin{figure}[htbp]
      \centering
      \includegraphics[width=0.8\linewidth]{Figure/admin_manage.png}
      \caption{The administrator's interface. (1) Button to enter the experiment. (2)Button to delete the experiment. (3) Button to download the experiment logs.}
      \label{Fig.manage}
    \end{figure}
\end{itemize}


% FYI ks checked up until here
\subsection{Technical Implementation}
\subsubsection{Collaborative Work}
To enable two Wizards to edit a document together and to collaborate on user speech and editing requests, it is important to choose an efficient and effective algorithm that avoids conflicts. This includes the operational transformation \cite{sun1998operational}, treeOPT (tree Operational Transformation) \cite{ignat2003customizable}. Finally, I chose the Conflict-free replicated data types (CRDT) \cite{shapiro2011conflict} algorithm because it can use mathematical models that usually do not involve index transformations, like linked Also, compared to OT, CRDT is more suitable for distributed systems, providing additional assurance that files can be synchronized with remote clients and do not require a central data source \cite{nicolaescu2016near}. In this case, we chose tiptap editor, which supports collaborative editor and is paired with Yjs, a framework that implements CRDT to achieve real-time common text editing using web-socket transmissions. At the same time, the Yjs web-socket will also transmit the location of each Wizards' "name flag" to another.

\subsubsection{System Architecture and Connection}
The Wizundry platform is a container-based system that includes the VueJs\footnote{See https://vuejs.org/} framework for the front-end, the Express\footnote{See https://expressjs.com/} framework for the NodeJs back-end server, the Yjs server and the MySQL database. The whole system is containerized by Docker\footnote{See https://www.docker.com/} and provided by docker-compose\footnote{See https://docs.docker.com/compose/} at Digital Ocean\footnote{See https://www.digitalocean.com/} cloud service provider to run on a remote Ubuntu server.

There are mainly two types of connection for the data transmission between server and client, which is the Web Socket Connection and the API Connection. There are two main types of connections for data transfer between the server and the client, namely web socket connections and API connections. In this system, considering the role-based and the need to transfer multiple forms of data, we use socket io as an alternative to the web socket provider. Although it is mentioned by Mike Pennisi \footnote{M. Pennisi, "Realtime node.js app: A stress testing story", [online] Available: https://bocoup.com/weblog/node-stress-test-analysis.} that Socket.io fallback to long polling is a really huge performance drawback. \cite{imre2016introduction} However, since it is unlikely that a large number of connections will be needed in a general WoZ experiment, it was decided to use this provider as the core technology to achieve collaborative work. On the other hand, for the Yjs Server, which is used to handle collaborative text and text cursor, I still used the traditional web socket technology and added a layer of optimized Yjs \footnote{Kevin, "Are CRDTs suitable for shared editing?", [online] Available: https://blog.kevinjahns.de/are-crdts-suitable-for-shared-editing/} framework to reduce the text latency between Wizard and user. The diagram (Fig.\ref{fig.architecture}) demonstrates the connection between each component and the technology used to implement it.
    \begin{figure}
      \centering
      \includegraphics[width=0.6\linewidth]{Figure/system-structure.png}
      \caption{The whole Wizundry System Architecture and Connection}
      \label{fig.architecture}
    \end{figure}


\subsubsection{Visual Components}
The interfaces of Wizundry is a front-end development framework using VueJs framework and Vuetify \footnote{See https://vuetifyjs.com/}, a material design framework. The platform panel style is done using some components that come with Vuetify. Using Vue as a framework is good because it is extensible, suitable for adding components according to different needs, and it also provides powerful router and state management features, \cite{wohlgethan2018supportingweb} makes Wizundry perfect Role-based rendering. And we also use tiptap2 as collaborative editor because she is a headless, framework-agnostic and extendable rich text editor, and experimenter can easily write plug-ins and load them into this editor according to their needs. She also fits perfectly with the Yjs framework and provides one of the fastest collaborative environments.


\subsection{Wizard Walk-through}
Multiple Wizards using with Wizundry platform has 4 steps:(1) Enter the experiment room, (2) Set up the feedback in advance, (3) Control the user's microphone, (4) Editing content, (5) Feedback to user.

\subsubsection{Step 1. Enter the experiment room}
The Wizundry platform is available directly cross-platform application. End-users can access the website directly through their browser to log in and use it. In particular, Wizundry allows the experimenter (admin) to select various types of features and then create multiple independent rooms (trials) for multiple Wizards to to conduct experiments simultaneously. Once Wizard has logged in, click on the corresponding room displayed on the landing page based on the trial ID. (Similar to Fig.\ref{Fig.manage}.1) The page will direct Wizards to the assigned experiment interface.

\subsubsection{Step 2. Set up the feedback in advance}
Wizundry allows multiple Wizards to customize the command boxes in advance and use it as a voice command in response to the user. The Wizard can fill in the "Command Boxes" to store text before the experiment starts (eg."Can you repeat again, please?").

\subsubsection{Step 3. Control the end-user's microphone}
The Wizundry platform allows multiple Wizards to operate the end-user's microphone simultaneously. When the microphone is turned on, the dictation system automatically transcribes all the end-user's speech directly into text and displays it in the collaborative editor (eg. "hair, em, hair cut, no,no,no, please change to the hairstyle"). When the microphone is turned off, stop dictation.

\subsubsection{Step 4. Editing content collaboratively}
The Wizard can manipulate text directly from the collaborative editor on the interface. Wizundry platform offers Wizards the ability to edit text together, for example by deleting or typing it directly. Multiple Wizards can see each other's editing text cursors and mouse cursors simultaneously. The Wizards need to follow the end-user's voice commands and do their best to modify the dictation of the text to the end-user's satisfaction.

\subsubsection{Step 5. Play the Feedback to end-user}
If Wizards encounter any issues during the end-user speech process, they can click on the play icon or use the "Enter" key and the text will be played directly to the end user via the Web Speech API (eg. "I got it" after user completes the composition).

==> findings.tex <==
\section{Findings}

We first present initial findings from the pilot study and the first formal experiments. We describe the revisions we subsequently made to Wizundry and the study procedure. We then present findings from the formal experiment.

\subsubsection{Feedback from the Pilot Study}
%In this study, 2 trials were performed in the [Single-Wizard] condition and 4 [Multi-Wizards].

Based on the pilot study, we added the [Multi-Cursor] function and improved the experimental workflow. We also identified a key challenge: \emph{search content that needs to be modified}. We observed that participants spent much time searching for text content that needed to be edited during the [Multi-Wizards] condition. The rhythm of cooperation within the dyad and the speed of task completion was disrupted because of this action. In the interview, participants generally reported that finding what the end-user needed to be modified was the most challenging operation. G1P2 mentioned, "I had to spend much time finding out what the user was saying before I could edit it. But I have not even found [the user] yet, and he is already moving on to the next composition." This was caused by the cognitive burden of having to make several decisions and actions at the same time in short succession. G2P2 said that "there was no time to think about using the 'Command Boxes' function".
Nevertheless, we found that with each dyad's agreed-upon division of labour, those who were not responsible for text editing sometimes could find the location more quickly. According to the video recordings, these Wizards dragged the mouse in response to the 'Search content' issues. In response to this strategy, we added a "Multi-cursor" function to Wizundry for the formal experiments. This feature allows participants to see each other's cursors on the screen.

We also improved the flow of the experiment based on feedback from participants and the end-user confederates. Instead of two trials, we had one trial in the [Single-Wizard] condition, since a second trial did not appear necessary for training and familiarization. We also modified the training session so that the experimenter carried out a few end-user tasks as a way of demonstrating the user-side interface to participants. We also added two performance criteria when instructing participants: 1) provide the best possible user experience for the end-user; and 2) optimize the cooperative process and try to find the best way of collaborating with their partner.

\subsubsection{Initial Feedback from the Formal Experiment}
%We conducted 1 trial in the [Single-Wizards] condition at first and then 4 trials in the [Multi-Wizards] in the study. We started with a user study of Group 3 and Group 4. 
In the first two sessions, we noticed several small design and technical issues that we corrected before the formal study. We changed the shortcut keys for the "Microphone" function in order to make it easier for users to switch on and off dictation. We also removed half of the "Command Boxes" from the system interface. 
%After completing the iterations of the system, we continued the experiment with the last two groups. 
During the subsequent training sessions, we emphasized the "line-break" feature to Group 5 and Group 6 and asked them whether they would like to use this feature in the formal trials. Depending on their choice, the experimenter controlled whether to turn off the "line-break" in their trials. No other changes were made.


\subsection{Multi-Wizard Cooperative Strategies}
The dyads of participants acting as Wizards were allowed to freely define and agree on a workable approach to the Wizardry based on their experiences in the single-person trial. We observed six types of cooperative strategies that can be divided by the division of work between the Wizards. Five dyads altered the way that they worked collaboratively over the course of the tria ls, while one dyad maintained the same approach from beginning to end. %In our study, we identified 6 types of Multi-Wizards collaborative strategies, depending on their different distribution of work. 
The strategies used in each dyad across trials and each Wizards operation are visualized in Fig.~\ref{fig.groupstrategy}.  We describe each strategy below.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=1\linewidth]{Figure/GroupStrategy_v1.png}
  \caption{(1) Group strategies for each of the [Multi-Wizard] condition trials; (2) Visualisation of Wizard operation in each trial;}
  \label{fig.groupstrategy}
\end{figure}

\subsubsection {Content-based} 
We observed G1 and G6 adopting this strategy, with participants separately responsible for each of the end-user's composed content and edited content. It was agreed between the participants that one would be primarily responsible for all of the user's content regarding Composition, while another would track the text that the user was Editing. This strategy appeared in the early trials (see G1T1, G6T2) and was used only once per dyad. 

We observed significant issues with "Microphone Control" when Wizards applied this strategy. In both dyads, there was no prior discussion about who would manage the microphone function, which resulted in all that the end-user said being dictated in the Content box. This may have led to confusion in the distribution of work. Participants commented that "the voice for composition and editing is not interrupted, and when the user speaks the system mixes all the content together, with repeats and overlays, making it very difficult to tell what to edit and what to [retain]. At this point the system is still dictating and the user keeps talking (G1P1)." G6P12 said "I had to think about what kind of content it was and then turn off the microphone, and there was not enough time."

\subsubsection {Interface-based}
Participants divided their roles based on the interface areas in which the Wizards worked. Participants were responsible for either the left or right side of the interface. The area on the left contains the "Microphone Control" and "Command Boxes" functions. The area on the right contains the full text editor or Content Box. We observed that G4 and G6 used this distribution of work for the task. G4 adopted this strategy after the first experiment, whereas G6 took it up for two continuous trials at the end (see G4T1, G6T3/T4).

\subsubsection {MicOnly-based}
In this strategy, one participant is responsible for the "Microphone Control" function only, and controls the timing of switching it on and off. The other participant is required to handle all of the rest of the work. This strategy was used continuously in the last three trials by both G3 and G4 until the end of the experiment (see G3T2/T3/T4,G4T2/T3/T4). We observed that the Wizard who was focused on controlling the microphone would perform work that had not been discussed in advance. G3P6, for instance, provided additional reminders to the other Wizard based on editing instructions issued by the user. This Wizard would proactively assist their teammate in finding the location of the text that the acting end-user needed to edit and provide the correct positioning information. They actively helped to remove extra dictation from the edit box, as well. 

\subsubsection {MicCommand-based}
This strategy involved one participant assigned to operate the "Microphone Control" and "Commands Box" functions, while the other assumed the rest of the work. This was the most frequently used strategy in our experiment. We found that the timing in terms of switching the microphone on and off was most precise for the dyads using this strategy. However, making edits was relatively slow. One notable example is G5, who did not change their strategy after it was established at the beginning of the experiment. However, they communicated most frequently during the experiment compared to other dyads. In particular, the participant who was primarily engaged in "Microphone" and "Commend Box" control also in parallel helped the other Wizard to locate edits. 

\subsubsection {Mix-based}
This strategy led to a process with less order. The allocation of work in the dyad was ambiguous and involved redundant working practices and ineffective results. It occurred in the last two trials of G2. We observed random jumps in the editing location of both participants and synchronized changes in the text. According to G2P4, who was originally working on the microphone, "I saw that [the other Wizard] was busy correcting something else and probably didn't notice, so I thought I would help him do it. But I thought it wasn't my job so I left it there." But his teammate commented, "I saw [the other Wizard's] edit cursor was in that spot and thought he would help me directly, but he stayed there. I was afraid we'd both change [something] at the same time." This shows that having unsaid expectations of each other may also be a cause of confusion. We discuss this in greater detail later on.
%(see 'Managing expectations and performance').

\subsubsection {Controller-based}
One dyad developed a strategy of dividing the labour by selecting which hardware devices each controlled (see G6T1). One Wizard operated the mouse only, while another focused on the keyboard. According to the interviews, the participants felt that focusing on one controller would reduce the burden of operation and improve efficiency. As G6P11 explained: "I can click several buttons with the mouse, so I don't have to press the keyboard with one hand and control the mouse at the same time."

\subsection{Attitudes towards Single-Wizard and Multi-Wizard Modes}
We mainly intended to explore whether or not the Wizundry system was effective at improving dictation work in a speech-based system using a Multi-Wizard setup. 
Some participants felt that multiple Wizards would be better (n=5). Multiple Wizards can be effective in solving the difficulties encountered in the single person mode. As well, some felt that a single Wizard was sufficient to control the task and that multiple Wizards were of limited benefit (n=4). Other participants who were in opposition to multiple Wizards felt that this extra person was very disruptive to individual play and could have a negative impact (n=3).
%the addition of a workforce when a Wizard is performing the task. And with this opportunity,
%We observed which cooperative strategies the participants generated when playing Wizards. 
Here, we consider participants' attitudes towards the [Single-Wizard] and [Multi-Wizards] conditions each experienced as a point of comparison.

\subsubsection{Multiple Wizards Are Better Than One}
In the observation and interviews, we found that participants felt adding one more Wizard can facilitate control of the system and accomplish the Wizard's goals. 
%Two Wizards result in a better outcome and greater efficiency, which can allow each to focus on their own tasks. 
As G3P5 said, "two Wizards [lead to] a better outcome and efficiency, which can let them focus on their own work." Some felt that adding a teammate reduced their workload by offloading tasks, especially helping them to control the microphone and by being able to use the 'Command Boxes' function. As G4P8 said, "I wouldn't have used the "Command Boxes" function before because I didn't have time to look at it. He [teammate] can use it to give feedback to users." Similar views were expressed by G6P11: "I wasn't sure I had edited according to the user's [requests] when I was alone before, and I didn't know if the user was happy with the result. If there were mistakes or uncertainties, I had to wait until the user checked and found them himself. But with an extra person helping me, I can use the Command function to check more often."

\subsubsection{Limited Benefits of Multi-Wizard}
Some participants felt that they were better off in the [Single-Wizard] condition, and did not feel that involving another Wizard helped.
%such as improving their task completion efficiency compared to [Multi-Wizards]. 
Even in the dyads with better outcomes, some participants felt that one Wizard was enough. However, considering user experience and speed, Multi-Wizard was superior. As G3P5 mentioned, "I can do the task when I'm by myself, and I don't feel special with an extra person. But with an extra person, it might increase the speed more." Others recognized that an extra Wizard reduced cognitive demand. As G5P9 stated, "I can concentrate on getting my work done and not have to think about so many things at once."

\subsubsection{Additional Wizards Are Redundant}
Some participants felt that the other Wizard was redundant, and that this affected their own performance. As G2P3 said, "I can do it myself. It's a waste of time when I have one more person to think about." 

\subsection{Dominant Personalities and Performance}
We found that the presence of a dominant Wizard reduced the occurrence of conflicts and led to both Wizards finishing the job efficiently. We observed that the dominant participant allocated the work distribution actively while the other Wizard acted as the copilot. In G3, G4, and G5, we found this dominant setup initiated by one of the participants.
These dominant Wizards communicated directly and maintained an efficient way of working during the experiment. The experimenter playing the role of the end-user noted that these dyads completed their tasks faster than other setups. This improved the end-user experience, especially in getting prompt feedback on the requests that they sent.  

Most dominant participants controlled the "Microphone" and spoke more. Without prior consultation, they were often able to quickly provide their teammates with a place to edit the text. As G4P8, a dominant Wizard, said, "I noticed that [the other Wizard] didn't seem to hear what the user had just said, so I reminded him." Similarly, G5P10 explained that "I saw that her cursor hadn't moved and guessed that she was still correcting the previous content or was searching for a location. I see it and I speak to her directly, so it's faster." We also observed "code-switching," where participants immediately switched from English to their native language to quickly pass on time-sensitive or complex information.
Non-native English-speaking dominant Wizards used direct prompts in their native Chinese language when they noticed that the other Wizard did not understand or did not respond to the end-user's instructions. These participants also used English to remind the other Wizard of proposed and selected content, while relaying end-user instructions in their native Chinese language.

\subsection {Attitudes towards System Features}
We interviewed participants about the features of the system that were observed to be least used as well as those that appeared to, but did not necessarily, aid collaboration.

\subsubsection{Command Boxes}
We observed that most participants (n=2) rarely used the "Command Boxes" function, even though they were responsible for controlling it. When difficulties were encountered, such as when the Wizard did not understand the end-user's instructions and were not able to complete their request in a timely manner, participants were still less likely to use the established feedback function. Some participants felt that they were in control of the task based on the end-user's instructions and therefore did not need to confirm with them. As G2P4 explained, "I can do everything myself very quickly, why do I need to communicate with the end-user?" When in solo mode, participants had no capacity to use the mouse to click on the play button. As G4P8 noted, "I'm already struggling to complete the task and don't have the extra power to think about using this feature." Some also felt that there were too many options in the Command Box. The Wizard was required to glance at the feedback text and skim-read it to use the feature, which was time-consuming. Meanwhile, the end-user may have already checked for themselves and given feedback on any errors or omissions. Hence there is no need for the Wizard to ask, leading to a feeling that the feature was unnecessarily.

\subsubsection{Line Break}
We developed a line break function to better support collaborative work between Wizards. We wanted each Wizard to be able to provide precise information about the position of certain text, such as the number of lines, to their partner via the "Line Break" function. But this was not as effective as we had expected. Observations and the interviews revealed several reasons for this. Each line contained a limited amount of content, such that each Wizard had to identify and piece together the information themselves. Additionally, splitting the composition into separate lines according to the duration of each pause led to more phrases in each line. Participants then needed to spend extra effort and time looking for components that could be pieced together into complete sentences and then doing the work of stitching these scattered components together. This was why G6 asked us to turn off this feature after the training session. G6P12 explained: "I have to count the lines and tell her. There is no serial number." G6P11 agreed: "Each line is not a complete sentence, so I have to look around to find out what is in a sentence and put it all together." When participants were asked about their experience with this feature, most were not aware of it, even though they had been trained to use this feature. This resulted in most participants simply not using it at all. Conversely, a few participants expressed the opposite attitude. For example, the G5 participants found this function extremely useful, especially for navigation of editing instructions from the end-user.

\subsubsection{Collaborative Cursor}
In response to feedback from G4, we added a synchronized cursor function to the main set of experiments. We had observed that participants often moved their cursor near to text that they then made the other Wizard aware of. We realized that it may be too time-consuming to find a given piece of text visually and then verbally relate this information to a partner. The purpose of the collaborative cursor was then to allow participants to see each other's mouse position in the interface, especially for directing their attention. However, some participants commented that the excessive number of icons on the interface, such as the text editing cursor and the roaming mouse icon, were distracting and hindered their ability to perform their tasks. As G6P12 said, "I don't like the big mouse. It moves around and always [steals my attention] when I'm doing text editing. And there's the cursor inside the text, and new text dictation keeps appearing."


\subsection{Workload Expectations and Actual Performance}
The relationship between actual and expected division of labour appeared to highly influence performance. Some dyads decided in the pre-experiment discussion to divide the labour in line with the MicCommand cooperative strategy. However, quantitative analysis of the logs indicated that the expected division of labour was not implemented (see G1 and G2 in Fig.~\ref{fig.groupstrategy}, where the circles represent the operation counts, including microphone and speaker control). In contrast, the data for the dyads that performed well and found the multi-Wizard context to be effective and effortless showed that their assigned work was almost identical to the actual results (see G3 and G5 in  Fig.~\ref{fig.groupstrategy}). The reason for not dividing the work as expected was to help the other Wizard finish tasks faster, but it led to an unclear division of labor and conflict.


\subsection{Cognitive Workload}

The raw, summed, and averaged NASA-TLX scores across participants for the dyad context are presented in Table~\ref{tab:nasatlx}. Participants in the [Multi-Wizard] condition had an overall average summed score of 31.9 (SD=7.1, MED=31, IQR=19) and mean score of 5.3 (SD=1.2, MED=5.2, IQR=3.2). With respect to the dyadic context, we noticed that some participants went out of their way to help their partner, but this was apparently disruptive rather than helpful.


\begin{table*}
  \caption{NASA-TLX scores for subjective workload.}
  \label{tab:nasatlx}
  \begin{tabular}{ccccccccccc}
    \toprule
    ID & Mental & Physical & Temporal & Perform. & Effort & Frust. & Sums & Means & St. Dev. & Inter. Q.\\
    \midrule
    1 & 9 & 7 & 8 & 5 & 8 & 8 & 45 & 7.5 & 2.5 & 4\\
    2&7&3&2&6&7&1&26&4.3&2.1&1.8\\
    3&10&1&8&4&10&8&41&6.8&2.2&2.3\\
    4&7&2&4&4&7&4&28&4.7&2.1&4.8\\
    5&7&8&3&9&6&3&36&6&1.4&2\\
    6&4&3&4&7&6&2&26&4.3&0.4&1\\
    7&5&5&5&5&6&5&31&5.2&2.6&4.5\\
    8&5&6&6&4&5&5&31&5.2&1.8&2.8\\
    9&4&4&5&7&3&1&24&4&1&1.8\\
    10&7&6&7&7&7&6&40&6.7&2.5&3.8\\
    11&5&3&6&9&5&3&31&5.2&1&1.5\\
    12&6&3&5&1&5&4&24&4&2.7&6.8\\
    \bottomrule
  \end{tabular}
\end{table*}




==> study.tex <==
\section{User Study: Using Wizundry to Understand the Multi-Wizard Experience}

We conducted a user study to refine the design of Wizundry as well as to better understand the multi-Wizard experience from the perspective of the Wizard. We were especially interested in cognitive workload, one of the key human factors hinted at in previous work. To this end, we 1) used a within-subjects design to compare Wizard behaviour in solo and multiple Wizard conditions; 2) observed the cooperative strategies that Wizards naturally employed while performing as a dyad; 3) assessed usability, UX, and subjective cognitive workload; and 4) employed a confederate end-user without the Wizards' knowledge as a measure of experimental control in terms of consistency across trials. %; and 3) tested using the Wizundry platform with 6 pairs of participants. 
We recruited a total of 12 participants who took on the role of the Wizard. Each participant experienced solo and multi-Wizard conditions. We first conducted a pilot study with 2 dyads of Wizards and then a formal study with 4 dyads of Wizards. After the pilot study, 
%and feedback from the experimental design implementation
we added a feature--keyboard shortcuts--and improved the system functionality (see Fig.~\ref{fig.trial_order}). Otherwise our approach in the pilots and formal experiments were identical. We detail below.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=1.0\linewidth]{Figure/TrialOrder_v2.png}
  \caption{Experiment trial order. The pilot study included G1/G1 and the formal study included G3/G4/G5/G6. EWC: Editing while composing; EAC: Editing after composing.}
  \label{fig.trial_order}
\end{figure}



%\hl{This allowed the remote experimenter to act as a user, dictate and edit the text on given scripts. Two Participants act the Wizards and need to simulate the intelligent dictation interface to handle the composing and editing of text simultaneously as requested by the user. Participants must use the Wizundry as a Wizard and provide a quality user experience until the user is satisfied with the content results presented in the system interface. Participants complete the individual tasks and then work in dyads to complete the same tasks. Participants need to consider and decide their working flow when they work together and communicate freely during the experiment. After finishing the tasks, they were asked to complete the NASA-TLX questionnaire and interviewed to provide feedback about user experience, System design, and collaborative strategies. There is no time limit for finishing a task.}


\subsection{Experimental Design}
The experimental design had one condition: Number of Users (Single-Wizard or Multi-Wizards). In the Single-Wizard or solo condition, one participant took on the role of a Wizard by themselves. Under the Multi-Wizards or dyad condition, two participants were randomly paired and asked to take on the role of Wizards at the same time. 

\subsection{Main Task}
The goal given to the Wizards was to provide the end-user with a great experience and avoid causing them frustration with the system. The main task was to use the Wizundry system to simulate an intelligent dictation interface by responding to the end-user's dictated speech and requests for text editing. In the Multi-Wizards condition, the Wizards needed to work together to decide on and optimize a collaborative approach to the Wizardry. They were given time to work out a plan before the end-user arrived. They were able to talk with each other before and during the main task.

On the end-user side, the main task was performed by a confederate, a researcher pretending to be an end-user. The confederate relied on prepared scripts for acting out the end-user dictation tasks, which required both composing and editing. These scripts used dialogue from established natural speech authoring actions, such as re-speaking and self-repair ~\cite{10.3115/981574.981581,liu2006enriching}. Based on the natural speech for dictation and text editing ~\cite{alto1989experimenting,ghosh2020commanding}, the scripts involved a combination of Editing after Composition (EAC) strategies and Editing while Composing (EWC) strategies. The confederate was trained and asked not to deviate from the scripts, so as to maintain a high degree of consistency across trials.
%The confederate end-user spoke it through the meeting application such as telephone call. 

\subsection{Equipment and Setting}
The experiment was conducted in a hybrid setting, a mix of online and offline modes, with the Wizard/s, the end-user confederate, and a remote experimenter in the same virtual meeting session. Zoom\footnote{https://zoom.us/} was used to allow the end-user confederate to be heard by the Wizards. The Wizard/s participated mainly offline, using separate computers (ThinkPad X390 laptops) in the same room as the "experimental" laptop (a 2019 13-inch MacBook Pro) that held the Zoom session with the end-user confederate. The Wizards were asked to disable their camera so as to maintain the illusion of interacting with a real end-user. Video and audio were taken using Zoom's recording features as well as screen recording software (screenshot toolbar on macOS and Windows). To reduce the risk of data loss caused by the network and/or software, each trial was also recorded with a voice recorder (Sony PCM-A10 Linear voice recorder).

\subsection{Participants}
We recruited 12 participants (4 women and 8 men) from the same local university to form 10 dyads. None had professional dictation training. All were non-native speakers and fluent in English, based on registration as full-time students in English-taught universities where their IELTS score needed to be at least 6.5. The trials were conducted in English. Participants had diverse backgrounds and education levels, holding bachelor, master, and doctoral degrees in computer science, communications, media, and art. Since the goal of our study was to refine the Wizundry system and evaluate the Wizard experience in a collaborative context, language fluency was not expected to be an influential variable.

\subsection{Procedure}
The experimenter first introduced the study and collected informed consent. The experimenter then confirmed the settings and operational status of the Wizundry system and Zoom with the Wizard participant/s. This involved checking the Zoom function settings, microphone channel, and status of Wizundry. To avoid the Wizard communicating directly with the end-user vocally, the microphone in Zoom was muted. The Wizard cold only hear the end-user's voice. Wizundry was used in full-screen mode. The participants began with a training session so as to get familiar with their role as Wizards, the interface of Wizundry, and the Wizundry task. Then they started the trials with a remote end-user confederate. Each trial required the completion of composing and editing one piece of text according to the acting end-user's script. Two EAC and EWC scripts were randomly chosen from the script repository and counterbalanced to ensure that different scripts were provided for each trial within one experiment (see Fig.~\ref{fig.trial_order}).

In the pilot study, participants (in G1 and G2) completed two [Single-Wizard] and four [Multi-Wizard] trials. In the formal study, participants (in G3-G6) completed one [Single-Wizard] trial and four [Multi-Wizard] trials.

The participant's goal was to edit the dictated/transcribed text to the (fake) end-user's satisfaction. Each participant began in the [Single-Wizard] condition and completed the tasks independently. After finishing the solo tasks, two participants from the same dyad were invited into the same Zoom room. They were tasked with using Wizundry together on their individual laptops. They could control the entire Wizundry system in a synchronized fashion. Before starting the [Multi-Wizard] condition, the two participants had to work together to come up with a feasible solution for working together as Wizards. They were allowed to discuss freely and modify their approach during the experiment. In all trials, they were allowed to take as long as needed to complete the task.

%We first conducted pilot studies with 2 dyads and then conducted formal experiments with 4 dyads. Based on participants' feedback and experience with the system in the pilot studies, we revised some of Wizundry's features. In the formal experiment, the functions of the iterations and updates in each step are described in detail in the following section. 
After finishing all trials, the experimenter conducted a semi-structured interview with each dyad and asked individual participants to fill in the NASA-TLX questionnaire. They were then thanked for their time and efforts. The experiment took around two hours for each dyad, with a break in the middle.

\subsection{Instruments}
Participants were given a questionnaire after the experiment with the NASA-TLX \cite{hart1988development} to evaluate subjective workload.

\subsection{Data Collection and Analysis}
The following data were collected: 1) screen recordings of participants and experimenters; 2) audio of participants' conversations throughout their experiments; 3) audio recordings of participants' interviews; 4) observations of experimenters during the process; 5) NASA-TLX self-reports; and 6) system log data, which logged the Wizard's usage of the Wizundry application components. We used both quantitative and qualitative analysis to analyse the corresponding data. Quantitative analysis was used for the operational log data recorded by the system. In line with Hart ~\cite{hart2006nasa}, we did not weight the NASA-TLX scores. Qualitative analysis was used to explore patterns in behaviours and attitudes in the observational and interview data. We used thematic analysis to group our findings under different categories.

